A Faster Tableau for CTL*

There have been several recent suggestions for tableau systems for deciding satisfiability in the practically important branching time temporal logic known as CTL*. In this paper we present a streamlined and more traditional tableau approach built upon the author's earlier theoretical work. Soundness and completeness results are proved. A prototype implementation demonstrates the significantly improved performance of the new approach on a range of test formulas. We also see that it compares favourably to state of the art, game and automata based decision procedures.

==> eptcsdata.tex <==
\providecommand{\firstpage}{50}
\providecommand{\publicationstatus}{Gabriele Puppis, Tiziano Villa (Eds.): Fourth International\\ Symposium on Games, Automata, Logics and Formal Verification\\
EPTCS 119, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.119.7}{10.4204/EPTCS.119.7}}

